Node Representation Learning for Directed Graphs

We propose a novel approach for learning node representations in directed graphs, which maintains separate views or embedding spaces for the two distinct node roles induced by the directionality of the edges. We argue that the previous approaches either fail to encode the edge directionality or their encodings cannot be generalized across tasks. With our simple \emph{alternating random walk} strategy, we generate role specific vertex neighborhoods and train node embeddings in their corresponding source/target roles while fully exploiting the semantics of directed graphs. We also unearth the limitations of evaluations on directed graphs in previous works and propose a clear strategy for evaluating link prediction and graph reconstruction in directed graphs. We conduct extensive experiments to showcase our effectiveness on several real-world datasets on link prediction, node classification and graph reconstruction tasks. We show that the embeddings from our approach are indeed robust, generalizable and well performing across multiple kinds of tasks and graphs. We show that we consistently outperform all baselines for node classification task. In addition to providing a theoretical interpretation of our method we also show that we are considerably more robust than the other directed graph approaches.

==> relatedwork.tex <==
\section{Related Work}
\label{sec:related-work}
We note that the focus of this work is learning unsupervised node representations and we therefore limit our related work discussion to unsupervised approaches.

\subsection{Directed Graph Embeddings.} 

Traditionally, undirected graphs have been the main use case for graph embedding methods. Manifold learning techniques \cite{NIPS2001_1961}, for instance, embed nodes of the graph while preserving the local affinity reflected by the edges. Chen et al.~\cite{chen2007directed} explore the directed links of the graph using random walks, and propose an embedding while preserving the local affinity defined by directed edges. Perrault-Joncas et al.~\cite{perrault2011directed} and Mousazadeh et al.~\cite{Mousazadeh:2015} learn the embedding vectors based on Laplacian type operators and preserve the asymmetry property of edges in a vector field.


\subsection{Shallow models for Node Embeddings.} 

Recent advances in language modeling and unsupervised feature learning in text inspired their adaptations~\cite{Grover:2016,Perozzi:2014,cao2015grarep, tang2015line} to learn graph embeddings. Though the text based learning methods \cite{mikolov2013distributed,pennington2014glove} inherently model neighborhood relations, a conceptual adaptation to graphs was required. \deepwalk~\cite{Perozzi:2014}, for instance, samples truncated random walks from the graph, thus treating \emph{walks} as equivalent of sentences, and then samples node-context pairs from a sliding window to train a \emph{Skip-Gram} model \cite{mikolov2013efficient, mikolov2013distributed}. The main idea is to relate nodes which can reach other similar nodes via random walks. \nodetovec \cite{Grover:2016}, on the other hand, uses a \emph{biased} random walk procedure to explore diverse neighborhoods.
\lineemb \cite{tang2015line} proposes objectives preserving the local pairwise proximity among the nodes (first-order proximity) and preserving the second-order proximity among nodes which share many neighbors. \verseemb \cite{tsitsulin2018verse} attempts to incorporate all the above ideas in one framework and proposes methods to preserve three similarity measures among nodes, namely Personalized PageRank, adjacency similarity and SimRank with the difference that it learns a single  embedding matrix as compared to node and context (usually discarded) matrices learnt by other methods.

\subsection{Deep Learning based Methods.}

Works such as \cite{Cao:2016,wang2016structural} investigate deep learning approaches for learning node representations. \cite{Cao:2016} first constructs a probabilistic co-occurence matrix for node pairs using a random surfing model. Instead of using SVD to obtain low-dimensional projections of this matrix, a stacked denoising autoencoder is introduced in the model to extract complex features and model non-linearities. \sdne \cite{wang2016structural} uses a multi-layer auto-encoder model to capture non-linear structures based on direct first- and second-order proximities. \cite{learnEdge2017} employs a deep neural network to learn asymmetric edge representations from trainable node embeddings. Like most of the other methods, it learns a single representation for a node, hence ignoring the asymmetric node roles. The downsides of these deep learning approaches, as compared to other approaches, are the computationally expensive optimization and elaborate parameter tuning resulting in very complex models. However, none of the above methods can preserve the asymmetry property in the embedding vector space of nodes, as by assigning a single representation to a node, they fail to preserve the role information of nodes and hence suffer from the limitations described earlier.


\subsection{Asymmetry preserving approaches} 

To the best of our knowledge, there are only two works~\cite{ou2016asymmetric,AAAI1714696} which learn and uses two embedding spaces for nodes, one representing its embedding in the source role and the other in the target role. 
Note that \cite{learnEdge2017} does not preserve asymmetry for the nodes, which is the main theme of this work (more comparisons and discussions on this method can be found in Section~\ref{sec:supplementary}). 
\hoppe~\cite{ou2016asymmetric} preserves the asymmetric role information of the nodes by approximating high-order proximity measures like Katz measure, Rooted PageRank etc. Basically they propose to decompose the similarity matrices given by these measures and use the two decompositions as representations of the nodes. To avoid the computation of the similarity matrices and high computation cost of SVD, they exploit an interesting general formulation of these similarity measures and compute a low rank factorization without actually creating the full similarity matrix. \hoppe cannot be easily generalized as it is tied to a particular measure. 
The authors in~\cite{AAAI1714696} propose \app proposes a random walk based method to encode rooted PageRank proximity. 
\app{} uses a directed walk like \cite{Grover:2016,Perozzi:2014} to sample node neighborhoods as training data. Specifically,it uses directed random walks with restarts to generate training pairs. Unlike other \deepwalk type random walk based methods, \app does not discard the learnt context matrix, on the other hand it uses it as a second (target) representation of the node. 
However, the random walk employed sometimes is unable to capture the global structure of the graph.
Consider a directed graph with prominent hub and authority structure where a lot of authority nodes have no outgoing links. In such a case any directed random walk from a source node will halt after a few number of steps, irrespective of the stopping criteria. 
% Consequently, the global structure of the directed graph remains unexplored using such walks.

In principle all other random based methods can also be modified by using the second learned context matrix as the second representation of the node. In essence, the neighborhood structure of a node explored by \app is similar to other random walk based methods. An exhaustive account of the various node embedding approaches can be found in these surveys~\cite{zhang2018network,cai2018comprehensive}.

We comment that because of use of term 'role' our work should not be confused with  role discovery in graphs \cite{henderson2012rolx} which deals with finding groups of nodes that share similar graph topological structure. 



